Neurosymbolic Methods for Dynamic Knowledge Graphs

Knowledge graphs (KGs) have recently been used for many tools and applications, making them rich resources in structured format. However, in the real world, KGs grow due to the additions of new knowledge in the form of entities and relations, making these KGs dynamic. This chapter formally defines several types of dynamic KGs and summarizes how these KGs can be represented. Additionally, many neurosymbolic methods have been proposed for learning representations over static KGs for several tasks such as KG completion and entity alignment. This chapter further focuses on neurosymbolic methods for dynamic KGs with or without temporal information. More specifically, it provides an insight into neurosymbolic methods for dynamic (temporal or non-temporal) KG completion and entity alignment tasks. It further discusses the challenges of current approaches and provides some future directions.

==> tex/LLMs-4-TKGC.tex <==
\section{Large Language Models for Temporal Knowledge Graph Completion}

This section only discusses about the capabilities of Large Language Models for the task of TKGC. %Non-Temporal DKG completio

==> tex/preliminaries.tex <==
\section{Preliminaries}\label{sec:prelimiaries}

%Terms Introduced
%Non-temporal
%we need to mention the term "versioning" for "snapshots"

%important to make a differentiation

%https://medium.com/@researchgraph/dynamic-knowledge-graphs-a-next-step-for-data-representation-c35a205a520a 

%\begin{definition}[Static Knowledge Graph]
%\label{def:triple-set}
%A knowledge graph is a directed, labeled graph $G=(V,E,l, L_G)$, with $V$ the set of nodes, $E$ the set of edges, $L_G$ the set of labels, and a mapping $l : V \cup E \rightarrow L_G$. A triple $t=(e_h,r,e_t)$ is a labelled edge, i.e., $(e_h,r,e_t)=(l(e_h), l(r), l(e_t))$ where $r \in E$ and $e_h, e_t \in V$.  
%\end{definition}


\begin{definition}[Static Knowledge Graph]
\label{def:triple-set}
Let $\mathcal{G}=(\mathcal{V},\mathcal{E},\mathcal{L})$ be a directed labeled graph, where $V$ is the set of entities, $\mathcal{E}$ the set of directed edges, and $\mathcal{L}$ the set of labels, and a mapping $l : \mathcal{V} \cup \mathcal{E} \rightarrow \mathcal{L}$. $ \mathcal{F} = \mathcal{E} \times \mathcal{V} \times \mathcal{E}$ represents a set of facts and $f =(e_h,r,e_t)$ where $f \in \mathcal{F}$ and $e_h,e_t \in \mathcal{E} $, $r \in \mathcal{V}$.  
\end{definition}


\begin{definition}[Static Knowledge Graph~\cite{DBLP:journals/kbs/WuKYQW22} (last version)]
    \label{def:skg}
    Let $\mathcal{G}=\{(h,r,t)\}\subseteq\mathcal{E}\times \mathcal{R}\times(\mathcal{E}\cup\mathcal{L})$ be a directed labeled graph, where $\mathcal{E}$ is the set of entities, $\mathcal{R}$ is the set of relations, and $\mathcal{L}$ is the set of literals.
    
    \noindent Each element $(h,r,t)$ represents a triple, where $h$ is the head (or subject), $r$ is the relation (or predicate, property, or edge), and $t$ is the tail (or object).
\end{definition}

\noindent Note that the tail can be an entity or a literal (e.g.,~a string, a date, an integer, etc.).


\begin{definition}[Static Knowledge (Optional)]
    Let $\mathcal{G}=(\mathcal{E},\mathcal{R},\mathcal{L}, \mathcal{T})$ be a directed labeled graph, where $\mathcal{E}$ is the set of entities, $\mathcal{R}$ is the set of relations, $\mathcal{L}$ is the set of literals, and $\mathcal{T} \subseteq \mathcal{E}\times \mathcal{R}\times(\mathcal{E}\cup\mathcal{L})$  is the set of facts or triples .
\end{definition}


%\gag{We may need to later edit the definition to separate the definition of relations into object properties and data properties because some KGC approaches differentiate them. But we can do this later of course.}

%\gag{If we go with Definition 3, we should use a different symbol/style for time stamp for the temporal KG Definition}



% \ph{We quickly discuss that but should we add literals? I would vote in favor except if literals are not used in the approaches described in the other sections.}\ma{I would wait until the end for that, in case we are discussing some methods that use literals.}

%\ph{I moved TKG before DKG since the latter is more generic than SKG and TKG} \ma{thanks}

\begin{definition}[Temporal Knowledge Graph (last version)]
Let $\mathcal{G} = (\mathcal{V},\mathcal{E},\mathcal{L},\mathcal{Q},\mathcal{T})$ be a directed labeled graph, where $\mathcal{E}$,$\mathcal{V}$, $\mathcal{L}$, and $\mathcal{T}$ are the set of entities, relations, labels, and timestamps respectively. $l : \mathcal{V} \cup \mathcal{E} \rightarrow \mathcal{L}$ defines a mapping of labels to the sets of entities and relations. A set of all possible facts is denoted as $ \mathcal{Q} \in \mathcal{E} \times \mathcal{V} \times \mathcal{E} \times \mathcal{T}$ and one fact is represented as $s = \{e_h,r,e_t,[\tau_s,\tau_e ]\}$ where $e_h,e_t \in \mathcal{E} $, $r \in \mathcal{V}$, and $\tau_s, \tau_e \in \mathcal{T}\cup \{\emptyset \}$ and $\tau_s$ and $\tau_e$ represent the start and end time, i.e., $\tau_s < \tau_e$ . If $\tau_s = \tau_e$ then it represents a point in time $\tau\in T$. %The $\tau_{\emptyset}$ represent the absence of the timestamp. \ma{add reference, point in time which is null to represent co-occurrence of non-temporal and temporal.} 
\end{definition}

We can now extend the definition of a static knowledge graph to a temporal knowledge graph, where each triple can have a time interval representing its temporal validity:
\begin{definition}[Temporal Knowledge Graph]
    \label{def:tkg}
    Let $\mathcal{G}=\{(h,r,t,[\tau_s,\tau_e])\}\subseteq\mathcal{E}\times \mathcal{R}\times(\mathcal{E}\cup\mathcal{L})\times\mathcal{T}^2$ be a directed labeled graph, where $\mathcal{E}$ is the set of entities, $\mathcal{R}$ is the set of relations, $\mathcal{L}$ is the set of literals, and $\mathcal{T}$ is the set of timestamps (including the empty timestamp).
    
    \noindent Each element $(h,r,t,[\tau_s,\tau_e])$ represents a quadruple, where $h$ is the head, $r$ is the relation, $t$ is the tail, and $\tau_s$ and $\tau_e$ represent the start and end time, i.e., the time interval during which the fact is valid.
\end{definition}
\noindent Note that if $\tau_s = \tau_e$, the time interval represents a point in time $\tau$. 
A time interval can also be empty, meaning that the fact is always valid or its temporal validity is unknown or not applicable.
Additionally, one of the two timestamps of an interval can be missing, meaning that a fact is true only up until (respectively after) a point in time.

\ph{TODO: explain what is the difference between a timestamp and a timestep -> the first refers to the validity of the fact, while the second is the date of the snapshot}

\ph{I tried something else for the definition of DKGs.}\ma{thank you for the reorganization :) looks good. I did think of delta at some point but in DL delta is used for interpretation ... but with a superscript.... we are losing the timestamp of triples. One snapshot can have triples with older timestamps}

\begin{definition}[Dynamic Knowledge Graph]
    A dynamic knowledge graph $\mathcal{G}$ is a sequence of directed labeled graphs $\{\mathcal{G}_{t_0}, \mathcal{G}_{t_1}, \ldots, \mathcal{G}_{t_n}\}$ indexed by time steps $t_0, t_1, \ldots, t_n$ such that $t_0 < t_1 < \cdots < t_n$. Each graph $\mathcal{G}_{t_i} = (\mathcal{V}_{t_i}, \mathcal{E}_{t_i}, \mathcal{L}_{t_i})$ at time step $t_i$ consists of:
    \begin{itemize}
        \item $\mathcal{V}_{t_i}$: the set of entities,
        \item $\mathcal{E}_{t_i}$: the set of relations,
        \item $\mathcal{L}_{t_i}$: the set of labels.
    \end{itemize}

    $\mathcal{T}$ is the set of all timestamps $t_0, t_1, \ldots, t_n$. The function $l: \mathcal{V}_{t_i} \cup \mathcal{E}_{t_i} \rightarrow \mathcal{L}_{t_i}$ maps entities and relations to their labels at time $t_i$.

    The graph $\mathcal{G}_{t_i}$ represents a snapshot of the dynamic graph $\mathcal{G}$ at time $t_i$. For any $t_i, t_{i-1} \in \mathcal{T}$, if $\mathcal{G}_{t_{i-1}} = (\mathcal{V}_{t_{i-1}}, \mathcal{E}_{t_{i-1}}, \mathcal{L}_{t_{i-1}})$ and $\mathcal{G}_{t_i} = (\mathcal{V}_{t_i}, \mathcal{E}_{t_i}, \mathcal{L}_{t_i})$, then:
    \begin{align*}
        \mathcal{V}_{t_i} & = \mathcal{V}_{t_{i-1}} \cup \mathcal{V^+} \setminus \mathcal{V^-} \quad \text{where } \Delta\mathcal{V} \text{ represents the changes in the set of entities},  \\
        \mathcal{E}_{t_i} & = \mathcal{E}_{t_{i-1}} \cup \Delta\mathcal{E} \quad \text{where } \Delta\mathcal{E} \text{ represents the changes in the set of relations}, \\
       l_{t_i}           & = l_{t_{i-1}} \cup \Delta l \quad \text{where } \Delta l \text{ maps the changes in entities and relations to labels in } \mathcal{G}_{t_i}.
    \end{align*}
    \ph{add facts, change edges. Try to make a general def working with SKG and TKG}
\end{definition}

\ph{should we integrate directly in the DKG definition the possibility to have an SKG or a TKG indifferently? That would mean adding an optional set of time intervals} \ma{I think so it completes the definition and possibilities}

\ma{Inspired by this - I finally found an article but it is still graphs and not knowledge graphs: \url{https://link.springer.com/chapter/10.1007/978-3-030-47426-3_32} }

\begin{definition}[Dynamic Knowledge Graph (last version)]
    A dynamic knowledge graph $\mathcal{G}$ is a sequence of knowledge graphs $\{\mathcal{G}_{t_0}, \mathcal{G}_{t_1}, \ldots, \mathcal{G}_{t_n}\}$ indexed by time steps $t_0, t_1, \ldots, t_n$ such that $t_0 < t_1 < \cdots < t_n$ and $\forall t_i, t_i\in\mathcal{T}$, where $\mathcal{T}$ is the set of all timestamps. 
    Each graph $\mathcal{G}_{t_i}$, at time step $t_i$, can be either:
    \begin{itemize}
        \item A static knowledge graph as defined in Definition~\ref{def:skg}, i.e., $\mathcal{G}_{t_i}=\{(h,r,t)\}\subseteq\mathcal{E}_{t_i}\times \mathcal{R}_{t_i}\times(\mathcal{E}_{t_i}\cup\mathcal{L}_{t_i})$.
        \item A temporal knowledge graph as defined in Definition~\ref{def:tkg}, i.e., $\mathcal{G}_{t_i}=\{(h,r,t,[\tau_s,\tau_e])\}\subseteq\mathcal{E}_{t_i}\times \mathcal{R}_{t_i}\times(\mathcal{E}_{t_i}\cup\mathcal{L}_{t_i})\times\mathcal{T}^2_{t_i}$.
    \end{itemize}
    The graph $\mathcal{G}_{t_i}$ represents a snapshot of the dynamic graph $\mathcal{G}$ at time $t_i$.

    The transition between two consecutive snapshots $\mathcal{G}_{t_{i-1}}$ and $\mathcal{G}_{t_i}$ can be characterized by changes in entities, relations, literals, and facts. 
    Formally:
    \begin{align*}
        \mathcal{E}_{t_i} & = \mathcal{E}_{t_{i-1}} \cup \mathcal{E}^{\text{+}}_{t_i} \setminus \mathcal{E}^{\text{-}}_{t_{i-1}} \quad \text{where } \mathcal{E}^{\text{+}}_{t_i} \text{ and } \mathcal{E}^{\text{-}}_{t_{i-1}} \text{ represent the additions and removals of entities}, \\
        \mathcal{R}_{t_i} & = \mathcal{R}_{t_{i-1}} \cup \mathcal{R}^{\text{+}}_{t_i} \setminus \mathcal{R}^{\text{-}}_{t_{i-1}} \quad \text{where } \mathcal{R}^{\text{+}}_{t_i} \text{ and } \mathcal{R}^{\text{-}}_{t_{i-1}} \text{ represent the additions and removals of relations}, \\
        \mathcal{L}_{t_i} & = \mathcal{L}_{t_{i-1}} \cup \mathcal{L}^{\text{+}}_{t_i} \setminus \mathcal{L}^{\text{-}}_{t_{i-1}} \quad \text{where } \mathcal{L}^{\text{+}}_{t_i} \text{ and } \mathcal{L}^{\text{-}}_{t_{i-1}} \text{ represent the additions and removals of literals}, \\
        \mathcal{G}_{t_i} & = \mathcal{G}_{t_{i-1}} \cup \mathcal{G}^{\text{+}}_{t_i} \setminus \mathcal{G}^{\text{-}}_{t_{i-1}} \quad \text{where } \mathcal{G}^{\text{+}}_{t_i} \text{ and } \mathcal{G}^{\text{-}}_{t_{i-1}} \text{ represent the additions and removals of facts}.
    \end{align*}
    
    Additionally, if $\mathcal{G}_{t_i}$ is a temporal knowledge graph, it can include changes in the temporal intervals of the quadruples.
\end{definition}

%\begin{definition}[Dynamic Knowledge Graph - 2]

%Let $G_{t_i} = (V,E,L,T)$ be a directed labeled graph, where $E$,$V$, $L$, and $T$ are the set of entities, relations, labels, and timestamps respectively. The function $l : V \cup E \rightarrow L$ defines a mapping of labels to the sets of entities and relations. $G_{t_i}$ represents the snapshot of the graph G at timestep $t_i$ where $t_0 < t_i < t_n$ or $i \in {0,1,\dots,n}$. If ($\forall \tau \in T,\tau = t_i) \Rightarrow (G_{t_i} = (V,E,L))$. 
    
%\end{definition}


%$\forall \tau \in T$ if $\tau = t_i$ then $G_{t_i} = (V,E,L)$ == ($\forall \tau \in T,$\tau = t_i$) \Rightarrow (G_b = (V,E,L))


%\ma{the time stamp t will overlap with the t of the tail so we should go for $e_h$ , $e_t$ for head and tail respectively and $r$ remains the same. Here $e_h,e_t \in \mathcal{E}$ I take care of the labels later.}. 

%\begin{definition}[Temporal Knowledge Graph]
%Let G = (E,V,T) be a directed labeled graph, where E,V, and T are the set of entities, relations, and timestamps respectively. A set of all possible facts is denoted as $ S \in E \times V \times E \times T$ and one fact is represented as $s = \{e_h,r,e_t,\tau\}$ where $e_h,e_t \in E $, $r \in V$, and $\tau \in T$. 
%\end{definition}

%https://arxiv.org/pdf/2309.16357v1 reference for temporality
%temporal knowledge graph: pseudo definition: https://arxiv.org/pdf/1705.05742 mehwish to prepare the definition of temporal kg

%Fabians recommended papers: https://suchanek.name/work/publications/aaaij.pdf , https://suchanek.name/work/publications/acm-csur-2023.pdf 
